LayoutGMN: Neural Graph Matching for Structural Layout Similarity

We present a deep neural network to predict structural similarity between 2D layouts by leveraging Graph Matching Networks (GMN). Our network, coined LayoutGMN, learns the layout metric via neural graph matching, using an attention-based GMN designed under a triplet network setting. To train our network, we utilize weak labels obtained by pixel-wise Intersection-over-Union (IoUs) to define the triplet loss. Importantly, LayoutGMN is built with a structural bias which can effectively compensate for the lack of structure awareness in IoUs. We demonstrate this on two prominent forms of layouts, viz., floorplans and UI designs, via retrieval experiments on large-scale datasets. In particular, retrieval results by our network better match human judgement of structural layout similarity compared to both IoUs and other baselines including a state-of-the-art method based on graph neural networks and image convolution. In addition, LayoutGMN is the first deep model to offer both metric learning of structural layout similarity and structural matching between layout elements.

==> LayoutGMN-CVPR'21/0-abstract.tex <==
\begin{abstract}
%As a fundamental representation in graphic and architectual designs, layouts are expressed by the arrangement of a set of semantic elements within a  boundary. 
We present a deep neural network to predict {\em structural similarity\/} between 2D layouts by leveraging Graph Matching Networks (GMN). Our network, coined LayoutGMN, learns the layout metric via neural graph matching, using an attention-based GMN designed under a triplet network setting. To train our network, we utilize weak labels obtained by pixel-wise Intersection-over-Union (IoUs) to define the triplet loss. Importantly, LayoutGMN is built with a structural bias which can effectively compensate for the lack of structure awareness in IoUs. We demonstrate this on two prominent forms of layouts, viz., floorplans and UI designs, via retrieval experiments on large-scale datasets. In particular, retrieval results by our network better match human judgement of structural layout similarity compared to both IoUs and other baselines including a state-of-the-art method based on graph neural networks and image convolution. In addition, LayoutGMN is the first deep model to offer both metric learning of structural layout similarity {\em and\/} structural matching between layout elements.
\end{abstract}


==> LayoutGMN-CVPR'21/1-intro.tex <==
\blfootnote{$^{\dagger}$ Corresponding Author:manyil@sfu.ca}

\section{Introduction}
\label{sec:intro}

Two-dimensional layouts are ubiquitous visual abstractions in graphic and architectural designs. They typically represent blueprints or conceptual sketches for such data as floorplans, documents, scene arrangements, and UI designs. Recent advances in pattern analysis and synthesis have propelled the development of generative models for layouts~\cite{gadi2020read,li2019layoutgan,zheng2019content,hu2020graph2plan,li2019grains} and led to a steady accumulation of relevant datasets~\cite{zhong2019publaynet,wu2019data,3DFRONT,zheng2020s3d}. Despite these developments however, there have been few attempts at employing a {\em deeply learned metric\/} to reason about layout data, e.g., for retrieval, data embedding, and evaluation. For example, current evaluation protocols for layout generation still rely heavily on segmentation metrics such as intersection-over-union (IoU)~\cite{hu2020graph2plan,manandharlearning} and human judgement~\cite{hu2020graph2plan,li2019grains}. 
%\rz{[More cites]}

The ability to compare data effectively and efficiently is arguably the most foundational task in data analysis. The key challenge in comparing layouts is that it is not purely a task of visual comparison --- it depends critically on inference and reasoning about {\em structures\/}, which are expressed by the semantics and organizational arrangements of the elements or subdivisions which compose a layout. Hence, none of the well-established image-space metrics, whether model-driven, perceptual, or deeply learned, are best suited to measure structural layout similarity. Frequently applied similarity measures for image segmentation such as IoUs and F1 scores all perform pixel-level matching ``in place'' --- they are not structural and can be sensitive to element misalignments which are {\em structure-preserving\/}. 
%
%After all, these measures are {\em not\/} designed to match the layout structures as characterized by element arrangements and relations.

% without taking into account the highly variable nature of the semantic entities (e.g., their boundaries as well as labels) and their relations within the layouts.}
% assume that the images are aligned, while aligning layouts under structural variation is a challenging problem on its own.
%
%~\matt{I'm not sure exactly what is meant by the statement ``IoUs assume the images are aligned''. Yes it's true the predicted rectangles are aligned with the input image, but that seems like a positive and necessary thing.}~\ms{Notion of alignment here may have several interpretations: geometric, semantic etc. -- should either clarify or trim (latter probably better if we don't explicitly show we handle `alignment' better)}

\begin{figure}[t!]
    \centering
    \includegraphics[width=0.99\linewidth]{Figures/teaser.png}
    \caption{LayoutGMN learns a structural layout similarity metric between floorplans and other 2D layouts, through {\em attention-based neural graph matching\/}. The learned attention weights (numbers shown in the boxes) can be used to match the structural elements.}
    \vspace{-1 em}
     \label{fig:teaser}
\end{figure}

In this work, we develop a deep neural network to predict structural similarity between two 2D layouts, e.g., floorplans or UI designs. We take a predominantly structural view of layouts for both data representation and layout comparison. Specifically, we represent each layout using a directed, fully connected graph over its semantic elements. Our network learns structural layout similarity via neural graph matching, where an {\em attention-based graph matching network\/}~\cite{li2019graph} is designed under a {\em triplet network\/} setting. The network, coined LayoutGMN, takes as input a triplet of layout graphs, composed together by one pair of anchor-positive and one pair of anchor-negative graphs, and performs intra-graph message passing and cross-graph information communication per pair, to learn a graph embedding for layout similarity prediction.
%
In addition to returning a metric, the attention weights learned by our network can also be used to match the layout elements; see Figure~\ref{fig:teaser}.

To train our triplet network, it is natural to consider human labeling of positive and negative samples. However, it is well-known that subjective judgements by humans over structured data such as layouts are often unreliable, especially with non-experts~\cite{zhang2010methodology, brants2000inter}. When domain experts are employed, the task becomes time-consuming and expensive~\cite{zhang2010methodology, brants2000inter,hripcsak2002reference,fort2009towards,kim2008corpus,wilbur2006new}, where discrepancies among even these experts
still remain~\cite{hripcsak2002reference}. In our work, we avoid this issue by resorting to {\em weakly supervised\/} training of LayoutGMN, which obtains positive and negative labels from the training data through thresholding using layout IoUs~\cite{manandharlearning}.

The motivations behind our network training using IoUs are three-fold, despite the IoU's shortcomings for structural matching. First, as one of the most widely-used layout similarity measures~\cite{manandharlearning,hu2020graph2plan}, IoU does have its merits. %Also, it is objective and does not suffer from inconsistency issues associated with human feedback. 
Second, IoUs are {\em objective\/} and much easier to obtain than expert annotations. Finally and most importantly, our network has a built-in inductive bias to enforce structural correspondence, via inter-graph information exchange, when learning the graph embeddings.
%\agp{
The inductive bias results from an attention-based graph matching mechanism, which learns structural matching between two graphs at the node level (Eq \ref{eqn:inter_graph}, \ref{eqn:attention_sum}). Such a {\em structural bias\/} can effectively compensate for the lack of structure awareness in the IoU-based triplet loss during training. In Figure~\ref{fig:struct_bias}, we illustrate the effect of this structural bias on the metric learned by our network. Observe that the last two layouts are more similar structurally than the first two. This is agreed with by our metric LayoutGMN, but not by IoU feedback.
%}
%

\begin{figure}[t!]
    \centering
    \includegraphics[width=\linewidth]{Figures/struct_bias_single_row.png}
    \caption{Structure matching in LayoutGMN ``{\em neutralizes\/}'' IoU feedback.
%Impact of the structure-oriented inductive bias introduced by neural graph matching in LayoutGMN; see Figure~\ref{fig:teaser}. 
In each example (left: floorplan; right: UI design), a training sample $N$ labeled as ``Negative" by IoU is more structurally similar to the anchor ($A$) than $P$, a ``Positive'' sample. With structure matching, our network predicts a smaller $A$-to-$N$ distance than $A$-to-$P$ distance in each case, which contradicts IoU.}
     \label{fig:struct_bias}
\end{figure}

%Once trained, inference by LayoutGMN is highly efficiently, achieving a $50\times$ speed-up over IoU.
%\ms{Report timings in result section to back this up.}
%
%\agp{
We evaluate our network on retrieval tasks over large datasets of floorplans and UI designs, via Precision@$k$ scores, and investigate the stability of the proposed metric by checking retrieval consistency between a query and its top-1 result, over many such pairs; see Sec.~\ref{sec:eval_metrics}.%}
% We also present the impact of node features on the performance of LayoutGMN. " Then applications....
Overall, retrieval results by LayoutGMN better match human judgement of structural layout similarity compared to both IoUs and other baselines including a state-of-the-art method based on graph neural networks~\cite{manandharlearning}.
%
Finally, we show a label transfer application for floorplans enabled by the structure matching learned by our network (Sec \ref{sec:application}). 

%\agp{Pointers for Richard -- Structured annotation tasks are difficult due to: 
%\begin{enumerate}
%    \item Unreliable responses from non-expert users 
%    \item Iterative, time-consuming and expensive, when domain experts 
%    \item Even on domain experts, annotator discrepancies can never be eliminated \cite{hripcsak2002reference}
%\end{enumerate}
%}


==> LayoutGMN-CVPR'21/2-related_work.tex <==
\section{Related Work}
\label{sec:rw}

\paragraph{Layout analysis.}
%
%A fundamental challenge in analysing layouts of Floorplans, Documents, 2D Indoor Scenes (top-view) and User-Interfaces (UI) is the highly variable nature of the semantic entities (boundaries) and their relations across the dataset. Very 
Early works \cite{o1995document, breuel2003high} on document analysis involved primitive heuristics to analyse document structures. Organizing a large collection of such structures into meaningful clusters requires a distance measure between layouts, which typically involved content-based heuristics \cite{ritchie2011d} for documents and constrained graph matching algorithm for floorplans \cite{wessel2008room}. An improved distance measure relied on rich layout representation obtained using autoencoders \cite{deka2017rico, liu2018learning}, operating on an entire UI layout. Although such models capture rich raster properties of layout images, layout structures are not modeled, leading to noisy recommendations in contextual search over layout datasets.
%~\matt{it seems okay if they are not explicitly accounted for. it's up to us to convince the reader that this lack of explicit accounting results in a lower quality result}.~\ms{+1}
 
\vspace{-1 em}

\paragraph{Layout generation.}
%
Early works on synthesizing 2D layouts relied on exemplars \cite{hurst2009review,kumar2011bricolage,swearngin2018rewire} and rule-based heuristics~\cite{o2014learning, tabata2019automatic}, and were unable to capture complex element distributions. The advent of deep learning led to generative models of layouts of floorplans \cite{wu2019data,hu2020graph2plan,chen2020intelligent,nauata2020house}, documents \cite{li2019layoutgan, gadi2020read, zheng2019content}, and UIs \cite{deka2017rico, dayama2020grids}. Perceptual studies aside, evaluation of generated layouts, in terms of diversity and generalization, has mostly revolved around IoUs of the constituent semantic entities \cite{li2019layoutgan, gadi2020read, hu2020graph2plan}. While IoU provides a visual similarity measure, it is expensive to compute over a large number of semantic entities, and is sensitive to element positions within a layout.
Developing a tool for structural comparison would perhaps complement visual features in contextual similarity search.
%Often times, two layouts could be more similar structurally than visually, and can provide useful information for a user/designer
%~\matt{I would avoid seeing this as a visual or structural similarity comparison. It is probably stronger if we try to phrase this as a tool for structural comparison, but suggest that both types of comparisons can be incorporated as separate features}~\ms{+1}. 
In particular, a learning-based method that compares layouts structurally can prove useful in tasks such as layout correspondence, component labeling and layout retargeting. We present a Layout Graph Matching Network, called LayoutGMN, for learning to compare two graphical layouts in a structured manner.

\vspace{-1 em}

\paragraph{Structural similarity in 3D.} 
%
Fisher et al.~\cite{fisher2011characterizing} develop Graph Kernels for characterizing structural relationships in 3D indoor scenes. Indoor scenes are represented as graphs, and the Graph Kernel compares substructures in the graphs to capture similarity between the corresponding scenes. A challenging problem of organizing a heterogeneous collection of such 3D indoor scenes was accomplished in \cite{xu2014organizing} by focusing on a subscene, and using it as a reference point for distance measures between two scenes. Shape Edit Distance, SHED, \cite{kleiman2015shed} is another fine-grained sub-structure similarity measure for comparing two 3D shapes. These works provide valuable cues on developing an effective structural metric for layout similarity. Graph Neural Networks (GNN) \cite{li2015gated, kipf2016semi, bronstein2017geometric, schlichtkrull2018modeling} model node dependencies in a graph via message passing, and are the perfect tool for learning on structured data. GNNs provide coarse-level graph embeddings, which, although useful for many tasks \cite{tripathi2019compact, ashual2019specifying, johnson2018image, khan2019graph}, can lose useful structural information in contextual search, if each graph is processed in isolation. We make use of Graph Matching Network \cite{li2019graph} to retain structural correspondence between layout elements.

\vspace{-1 em}

\paragraph{GNNs for structural layout similarity.}
%
To the best of our knowledge, the recent work by Manandhar et al.~\cite{manandharlearning} is the first to leverage GNNs to learn structural similarity of 2D graphical layouts, focusing on UI layouts with rectangular boundaries. They employ a GCN-CNN architecture on a graph of UI layout {\em images\/}, also under an IoU-trained triplet network \cite{hoffer2015deep}, but obtain the graph embeddings for the anchor, positive, and negative graphs independently. %, through weak supervision using layout IoUs.

In contrast, LayoutGMN learns the graph embeddings in a {\em dependent\/} manner. Through cross-graph information exchange, the embeddings are learned in the context of the anchor-positive (respectively, the anchor-negative) pair. This is a critical distinction to GCN-CNN~\cite{manandharlearning}, while both train their triplet networks using IoUs. However, since IoU does not involve structure matching, it is not a reliable measure of structural similarity, leading to labels which are considered ``structurally incorrect"; see Figure~\ref{fig:struct_bias}.

In addition, our network does not perform any convolutional processing over layout images; it only involves eight MLPs, placing more emphasis on learning finer-scale structural variations for graph embedding, and less on image-space features. We clearly observe that the cross-graph communication module in our GMNs does help in learning finer graph embeddings than the GCN-CNN framework~\cite{manandharlearning}.
%
Finally, another advantage of moving away from any reliance on image alignment is that similarity predictions by our network are more robust against highly varied, non-rectangular layout boundaries, e.g., for floorplans.

%\matt{I'm not sure we should emphasize this until the user has cause to believe it. After all, convolutional approaches are very successful, and one might expect convolutional features to assist in matching the elements being compared. If I was comparing the layout of two 3D scans, I would hope that we would both use 3D convolutional features as well as structural features.  I think we need to give them more specifics on the layouts we are comparing to convince them that it's a good thing that we aren't performing any convolutional processing over the images. I think at this point it's not even obvious our method should be restricted to images as opposed to graphs}. 


==> LayoutGMN-CVPR'21/3-method.tex <==
\section{Method}
\label{sec:method}

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{Figures/fp_plus_layout_graph_rz}
    \caption{Given an input floorplan image with room segmentations in (a), we abstract each room into a bounding box and obtain layout features from the constituent semantic elements, as shown in (b). These features form the initial node and edge features (Section \ref{sec:layout_graph_extraction}) of the corresponding layout graph shown in (c).}
    \label{fig:layout_graph}
    \vspace{-1 em}
\end{figure}

The Graph Matching Network (GMN) \cite{li2019graph} consumes a pair of graphs, processes the graph interactions via an attention-based cross-graph communication mechanism and results in graph embeddings for the two input graphs, as shown in Fig \ref{fig:GMN}. %Unlike in GNNs \cite{li2015gated, bronstein2017geometric, schlichtkrull2018modeling} where a latent space embedding is obtained for individual graphs, GMNs are designed to output graph embeddings in the context of another graph. 
Our LayoutGMN plugs in the Graph Matching Network into a Triplet backbone architecture for learning a (pseudo) metric-space for similarity on 2D layouts such as floorplans, UIs and documents. 
%\matt{I don't think Floorplans and Documents should be capitalized, but I'm not very concerned one way or the other.}


\begin{figure}
    \centering
%    \includegraphics[width=\linewidth, height = 0.55\linewidth]{Figures/architecture.pdf}
    \includegraphics[width=\linewidth]{Figures/architecture.pdf}
    \caption{LayoutGMN takes two layout graphs as input, performs intra-graph message passing (Eq. \ref{eqn:intra_graph}), along with cross-graph information exchange (Eq. \ref{eqn:inter_graph}) via an attention mechanism (Eq. \ref{eqn:attention}, also visualized in Figure \ref{fig:teaser}) to update node features, from which final graph embeddings are obtained (Eq. \ref{eqn:aggregator_MLP}).}
    \label{fig:GMN}
    \vspace{-1 em}
\end{figure}


\subsection{Layout Graphs}
\label{sec:layout_graph_extraction}
Given a layout image of height $H$ and width $W$ with semantic annotations, we abstract each element into a bounding box, which form the nodes of the resulting layout graph. Specifically, for a layout image $I_1$, its layout graph $G_l$ is given by $G_l = (V, E)$, where the node set $V = \{\boldsymbol{v_1, v_2, ..., v_n}\}$ represents the semantic elements in the layout, and $E = \{\boldsymbol{e_{12}, ..., e_{ij}, .., e_{n(n-1)}}\}$, the edge set, represents the set of edges connecting the constituent elements. Our layout graphs are directed and fully-connected. %(see Section \ref{sec:full_vs_adj_graphs} for adjacency graphs).

%Two nodes in a graph are connected based on their proximity, i.e., there exists an edge between two nodes (layout elements) if they are placed within a certain distance threshold in the layout image. %\matt{We've discussed images before, but need to better describe at some point how we are going to process images into graphs.}\ms{We should have concrete examples of what a node represents and what an edge represents (not same as formalism below). Also, do all graphs have to be fully connected?}
%\vspace{-1.5 em}

\vspace{-10pt}

\paragraph{Initial Node Features.} There exist a variety of visual and content-based features that could be incorporated as the initial node features; ex. the text data/font size/font type of an UI element or the image features of a room in a floorplan. For structured learning tasks as ours, we ignore such content-based features and only focus on the box abstractions. Specifically, similar to \cite{gadi2020read, guo2019aligning}, the initial node features contain {\em semantic\/} and {\em geometric\/} information of the layout elements. As shown in Fig \ref{fig:layout_graph}, for a layout element $k$ centered at ($x_k, y_k$), with dimensions ($w_k, h_k$), its geometric information is:
\begin{equation*}
    \label{eqn:node_geo_vec}
    g_{k} = \left[\frac{x_k}{W}, \frac{y_k}{H}, \frac{w_k}{W},
    \frac{h_k}{H}, \frac{w_k h_k}{\sqrt{WH}}\right].
\end{equation*}
%\matt{It's a bit of a jump to go straight to this restriction. What about all the details contained in the nodes? Perhaps we are comparing UI elements each of which has an image or a label, it seems like there are a lot of other features available beyond the ones in this list in many cases and we should motivate our decisions as well as make it clear one could use other features.}
%\ms{Agreed completely, need to justify feature choice here relative to alternatives. Easiest would be to say `many options, here are some, we choose these and the rest are interesting but not our focus'.}
%As is common in natural language processing, 
Instead of one-hot encoding of the semantics, we use a learnable embedding layer to embed a semantic type into a 128-D code, $s_{k}$. A two-layer MLP embeds the 5$\times$1 geometric vector $g_{k}$ into a 128-D code, and is concatenated with the 128-D semantic embedding $s_{k}$ to form the initial node features $U = \{\boldsymbol{u_1, u_2, ..., u_n}\}$.

\vspace{-1.2em}
\paragraph{Initial Edge Features.} In visual reasoning and relationship detection tasks, edge features in a graph are designed to capture relative difference of the abstracted semantic entities (represented as nodes) \cite{guo2019aligning, yao2018exploring}. Thus, for an edge $e_{ij}$, we capture the spatial relationship (see Fig \ref{fig:layout_graph}) between the semantic entities by a 8$\times$1 vector:
\begin{equation*}
    \label{eqn:edge_vec}
    %\begin{aligned}
    \boldsymbol{e}_{ij} = \left[\frac{\Delta x_{ij}}{\sqrt{A_i}},
    \frac{\Delta y_{ij}}{\sqrt{A_i}}, \sqrt{\frac{A_j}{A_i}}, U_{ij},
    \frac{w_i}{h_i}, \frac{w_j}{h_j},\frac{\sqrt{\Delta x^2 + \Delta y^2}}{\sqrt{W^2 + H^2}}, \theta \right],
    %\end{aligned}
\end{equation*}
%\matt{similar comments for the node features above. These features are fine but we need to provide visual and qualitative examples beforehand to make it clear what we are trying to capture here, and acknowledge that in some cases we might have more information available.}
%\ms{+1}
where $A_{i}$ is the area of the element box $i$; $U _{ij}$ = $\frac{B{_i} \cap B_{j}}{B_{i}\cup B_{j}}$ is the IoU of the bounding boxes of the layout elements $i,j$;
$\theta = atan2(\frac{\Delta y}{\Delta x})$ is the relative angle between the two components, $\theta \in [-\pi,\pi]$; $\Delta x_{ij} = x_{j}-x_{i}$ and $\Delta y_{ij} = y_{j}-y_{i}$. This edge vector accounts for the translation between the two layout elements, in addition to encoding their box IoUs, individual aspect ratios and relative orientation. %However, in the case of Indoor Scenes, this edge vector is different as there is a lack of global alignment between the 3D scenes. Write here the edge vector used in the context of indoor scenes (TO-DO)

\subsection{Graph Matching Network}
\label{GMN}
The graph matching module employed in LayoutGMN is made up of three parts: (1) node and edge encoders, (2) message propagation layers and (3) an aggregator.

\vspace{-1 em}
\paragraph{Node and Edge Encoders.} We use two MLPs to embed the initial node and edge features and compute their corresponding code vectors:
\begin{equation}
\label{eqn:node_edge_mlps}
\begin{aligned}
  \boldsymbol{h_{i}}^{(0)} = MLP_{node}(\boldsymbol{u_{i}}), \forall i \in U \\
  \boldsymbol{r_{ij}} = MLP_{edge}(\boldsymbol{e_{ij}}), \forall (i,j) \in E
\end{aligned} 
\end{equation}
The above MLPs map the initial node and edge features to their 128-D code vectors.
%\matt{is this different than the MLP we just described in section 3.1?}

\vspace{-1em}
\paragraph{Message Propagation Layers.}
The graph matching framework hinges on coherent information exchange between graphs to compare two layouts in a structural manner. The propagation layers update the node features by aggregating messages along the edges within a graph, in addition to relying on a graph matching vector that measures how similar a node in one layout graph is to one or more nodes in the other. Specifically, given two node embeddings $\boldsymbol{h}_{i}^{(0)}$ and $\boldsymbol{h}_{p}^{(0)}$ from two different layout graphs, the node updates for the node $i$ are given by:
\begin{equation}
    \label{eqn:intra_graph}
    \boldsymbol{m}_{j\to i} = f_{intra}\left(\boldsymbol{h}_{i}^{(t)}, \boldsymbol{h}_{j}^{(t)}, \boldsymbol{r}_{ij}\right),  \forall (i,j) \in E_{1}
\end{equation}
\vspace{-1 em}
\begin{equation}
    \label{eqn:inter_graph}
    \boldsymbol{\mu}_{p\to i} = f_{cross}\left(\boldsymbol{h}_{i}^{(t)}, \boldsymbol{h}_{p}^{(t)}\right),  \forall i \in V_{1},   p \in V_{2}
\end{equation}
\vspace{-0.6 em}
\begin{equation}
    \label{eqn:node_update}
    \boldsymbol{h}_{i}^{(t+1)} = f_{update}\left( \boldsymbol{h}_{i}^{(t)}, \sum_{j} \boldsymbol{m}_{j\to i}, \sum_{p} \boldsymbol{\mu}_{p\to i}\right) 
\end{equation}

where $f_{intra}$ is an MLP on the initial node embedding code that aggregates information from other nodes within the same graph, $f_{cross}$ is a function that communicates cross-graph information, and $f_{update}$ is an MLP used to update the node features in the graph, whose input is the concatenation of the current node features, the aggregated information from within, and across the graphs. $f_{cross}$ is designed as an Attention-based module:

\begin{equation}
\label{eqn:attention}
\begin{aligned}
    a_{p \to i} = \frac{\exp(s_{h}( \boldsymbol{h}_{i}^{(t)}, \boldsymbol{h}_{p}^{(t)})}{\sum_{p} \exp(s_{h}( \boldsymbol{h}_{i}^{(t)}, \boldsymbol{h}_{p}^{(t)})} \\
    \boldsymbol{\mu}_{p\to i} = a_{p \to i}\left(\boldsymbol{h}_{i}^{(t)} - \boldsymbol{h}_{p}^{(t)}\right)
\end{aligned}  
\end{equation}
where $a_{p \to i}$ is the attention value (scalar) between node $p$ in the second graph and node $i$ in the first, and such attention weights are calculated for every pair of nodes across the two graphs; $s_{h}$ is implemented as the dot product of the embedded code vectors. The interaction of all the nodes $p \in V_{2}$ with the node $i$ in $V_{1}$ is then given by:
\begin{equation}
\label{eqn:attention_sum}
\sum_{p} \boldsymbol{\mu}_{p\to i} = \sum_{p} a_{p \to i}\left(\boldsymbol{h}_{i}^{(t)} - \boldsymbol{h}_{p}^{(t)}\right) = \boldsymbol{h}_{i}^{(t)} - \sum_{p} a_{p \to i}\boldsymbol{h}_{p}^{(t)}
\end{equation}

Intuitively, $\sum_{p} \boldsymbol{\mu}_{p\to i}$ measures the (dis)similarity between $\boldsymbol{h}_{i}^{(t)}$ and its nearest neighbor in the other graph. The pairwise attention computation results in stronger structural bonds between the two graphs, but requires additional computation. We use five rounds of message propagation, then the representation for each node is updated accordingly. 

\vspace{-1em}
\paragraph{Aggregator.}
A 1024-D graph-level representation, $\boldsymbol{h}_{G}$, is obtained via a feature aggregator MLP, $f_{G}$, that takes as input, the set of node representations $\{\boldsymbol{h}_{i}^{(T)}\}$, as given below:
\vspace{-0.6em}
\begin{equation}
\label{eqn:aggregator_MLP}
\boldsymbol{h}_{G} = MLP_{G}\left(\sum_{i\in V} \sigma(MLP_{gate}(\boldsymbol{h}_{i}^{(T)})) \odot MLP(\boldsymbol{h}_{i}^{(T)}) \right)
\end{equation}

Graph-level embeddings for the two layout graphs is similarly computed.
\begin{equation*}
\label{eqn:two_graph_embeddings}
\begin{aligned}
\boldsymbol{h}_{G_1} = f_{G}(\{\boldsymbol{h}_{i}^{(T)}\}_{i \in V_{1}})\\
\boldsymbol{h}_{G_2} = f_{G}(\{\boldsymbol{h}_{p}^{(T)}\}_{p \in V_{2}})
\end{aligned}
\end{equation*}


\subsection{Training}
\label{training}

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{Figures/triplet_backbone.png}
    \caption{Given a triplet of graphs $G_{a}$, $G_{p}$ and $G_{n}$ corresponding to the anchor, positive and negative examples respectively, the anchor graph paired with each of other two graphs is passed through a Graph Matching Network (Fig \ref{fig:GMN}) to get two 1024-D embeddings. Note that the anchor graph has different contextual embeddings $\boldsymbol{h}_{Ga}$ and $\boldsymbol{h'}_{Ga}$. LayoutGMN is trained using the margin loss (margin=5) on the $L_{2}$ distances of the two paired embeddings.}
    \label{fig:triplet_setting}
    \vspace{-1 em}
\end{figure}

To learn a layout similarity metric, we borrow the Triplet training framework \cite{hoffer2015deep}. Specifically, given two pairs of layout graphs, i.e., anchor-positive and anchor-negative, each pair is passed through the same GMN module to get the graph embeddings in the context of the other graph, as shown in Fig \ref{fig:triplet_setting}. A margin loss based on the $L_{2}$ distance between the graph embeddings, as given in equation \ref{eqn:margin_loss}, is used to backpropagate the gradients through GMN.
\begin{equation}
\label{eqn:margin_loss}
\begin{aligned}
L_{tri}(a,p,n) = max(0, \gamma + \left\|\boldsymbol{h}_{G_a}-\boldsymbol{h}_{G_p}\right\|_{2}\\
-\left\|\boldsymbol{h'}_{G_a}-\boldsymbol{h}_{G_n}\right\|_{2})
\end{aligned}
\end{equation}
%Next, write about how the triplets are obtained. Probably also check for changing the graph representation from euclidean space to Hamming space

==> LayoutGMN-CVPR'21/4-datasets.tex <==
\section{Datasets}
\label{sec:dataset}

We use two kinds of layout datasets in our experiments: (1) UI layouts from the RICO dataset \cite{deka2017rico}, and (2) floorplans from the RPLAN dataset \cite{wu2019data}. After some data filtering %\ms{refer to supplement for details?}
, the size of the two datasets is respectively, 66261 and 77669.
%\vspace{-1.5 em}
%\paragraph{Training Triplets.}
%In triplet learning, training triplets are either selected from a ground truth label set or are obtained via crowdsourcing. 

In the absence of a ground truth label set and the need for obtaining the triplets in a consistent manner, we resort to using IoU values of two layouts, represented as multi-channel images, to ascertain their closeness. Given an anchor layout, the threshold on IoU values to classify another layout as positive, from observations, is 0.6 for both UIs and floorplans. Negative examples are those that have a threshold value of at least 0.1 less than the positive ones, avoiding some incorrect "negatives" during training. 
%\matt{reviewers are going to point out that we claimed IoU wasn't the best option here, and we are training explicitly on that, so perhaps the best we could hope for is to achieve the metric that we said was not very good for this task.}
%\ms{+1 for above. Results could support this choice if we show that we end up significantly outperforming a naive IoU baseline.}
The train-test sizes for the aforementioned datasets are respectively: 7,700-1,588, 25,000-7,204. 
%\matt{I would move the triplet network architecture into the end of section 3.} 
In the filtered floorplan training dataset \cite{wu2019data}, the distinct number of semantic categories/rooms across the dataset is nine and the maximum number of rooms per floorplan is eight. Similarly, for the filtered UI layout dataset \cite{deka2017rico}, the number of distinct semantic categories is twenty-five and  the number of elements per UI layout across the dataset is at most hundred. 


==> LayoutGMN-CVPR'21/5-results_and_eval.tex <==
\section{Results and Evaluation}
\label{sec:results_eval}

We evaluate LayoutGMN by comparing its retrieval results to those of several baselines, evaluated using
human judgements. Similarity prediction by our network is efficient: taking ~33 milliseconds per layout pair on a CPU. With our learning framework, we can efficiently retrieve multiple, sorted results by batching the database samples.

\begin{figure*}[!t]
\centering
\includegraphics[width=\linewidth]{Figures/all_results.pdf}
\vspace{-0.5em}
\caption{Top-5 retrieved results for an input query based on IoU metric, GCN-CNN$\_$Triplet \cite{manandharlearning} and LayoutGMN. We observe that the ranked results returned by LayoutGMN are closer to the input query than the other two methods, although it was trained on triplets computed using the IoU metric. Attention weights for understanding structural correspondence in LayoutGMN are shown in Figure \ref{fig:teaser} and also provided in the supplementary material. UI and floorplan IDs from the RICO dataset \cite{deka2017rico} and RPLAN dataset \cite{wu2019data}, respectively, are indicated on top of each result. More results can be found in the supplementary material.}
\label{fig:ui_fp_rets}
\end{figure*}

\subsection{Baselines}
\label{sec:baseline_comparisons}

%There are several existing methods that can be used to evaluate structural similarity. We start by summarizing the technical details of these baselines.

\paragraph{Graph Kernel (GK) \cite{fisher2011characterizing}.}
%\textbf{Graph Kernel (GK) \cite{fisher2011characterizing}}: 
GK is one of the earliest structural similarity metrics, initially developed to compare indoor 3D scenes. We adopt it to 2D layouts of floorplans and UI designs. We input the same layout graphs to GK to get retrievals from the two databases, and use the best setting based on result quality/computation cost trade-off. %The walk-length used is 4 in the case of floorplans and 2 for UI layouts, mainly due to the computation cost/result quality trade-off based on the number of semantic elements (upto 8 elements per floorplan vs. upto 100 per UI layout). \matt{we don't need to give this much detail here since we aren't proposing the method, we could just say ``which empirically gave the best results for each category.''}

\vspace{-10pt}

\paragraph{U-Net \cite{ronneberger2015u}.}
%\textbf{U-Net \cite{ronneberger2015u}}: 
As one of the best segmentation networks, we use U-Net %with the same parameter setting as in Pytorch, 
in a triplet network setting to auto-encode layout images. The input to the network is a multi-channel image with semantic segmentations. The network is trained on the same set of triplets as LayoutGMN until convergence. %\matt{Perhaps ``we use the default U-Net parameters from PyTorch'' or something to be more specific than ``uNet''}
%\textbf{CAE}: We use a con

\vspace{-10pt}

\paragraph{IoU Metric.}
%\textbf{IoU Metric}: 
Given two multi-channel images, we use the IoU values between two layout images to get their IoU score, and use this score to sort the examples in the datasets to rank the retrievals for a given query.

\vspace{-10pt}

\paragraph{GCN-CNN \cite{manandharlearning}.}
%\textbf{GCN-CNN \cite{manandharlearning}}: 
The state-of-the-art network for structural similarity on UI layouts is a hybrid network comprised of an attention-based GCN, similar to the gating mechanism in \cite{li2015gated}, coupled with a CNN. In this original GCN-CNN, the training triplets are randomly sampled every epoch, leading to better training due to diverse training data. In our work, for a fair comparison over all the aforementioned networks, we sample a fixed set of triplets in every epoch of training. The GCN-CNN network is trained on the two datasets of our interest, using the same training data as ours.

Qualitative retrieval results for GCN-CNN, IoU metric and LayoutGMN for a given query are shown in Figure \ref{fig:ui_fp_rets}.
\input{Tables/precision_scores_table}

\subsection{Evaluation Metrics}
\label{sec:eval_metrics}

%\vspace{-15pt}

\paragraph{\emph{Precision@k} scores.}
%\textbf{\emph{Precision@k} scores}: 
To validate the correctness of LayoutGMN as a tool for measuring layout similarity, we start by evaluating layout retrieval from a large database. A standard evaluation protocol for the relevance of ranked lists is the {\em{Precision@k}\/} scores \cite{manning2008evaluation}, or \emph{P@k}, for short. Given a query $q_{i}$ from the query set $Q = \{q_{1}, q_{2}, q_{3}, ..., q_{n}\}$, we measure the relevance of the ranked lists $L(q_{i}) = [l_{i1}, l_{i2},...., l_{ik}, ....]$ using the precision score, % defined as:
%
%Specifically, given a query $q_{i}$ from a query set $Q = \{q_{1}, q_{2}, q_{3}, ..., q_{n}\}$, we measure the relevance of the ranked lists $L(q_{i}) = [l_{i1}, l_{i2},...., l_{ik}, ....]$ returned by LayoutGMN. A standard evaluation protocol for measuring the relevance of ranked lists is the {\em{Precision@k}\/} scores \cite{manning2008evaluation}, and is defined as:
%
\begin{equation}
\label{eqn:precision_formula}
P@k(Q,\emph{L}) = \frac{1}{k|Q|} \sum_{q_{i} \in Q} \sum_{j=1}^{k} \emph{rel}(L_{ij}, q_{i}),
\end{equation}
where \emph{rel}($L_{ij}$, $q_{i}$) is a binary indicator of the relevance of the returned element $L_{ij}$ for query $q_{i}$. 
In our evaluation, due to the lack of a \emph{labeled} and \emph{exhaustive} recommendation set for any query over the layout datasets employed, such a binary indicator is determined by human subjects. 

Table \ref{tab:precision_scores} shows the  \emph{P@k} scores for different networks described in Section \ref{sec:baseline_comparisons} employed for the layout retrieval task. To get the precision scores, similar to \cite{manandharlearning}, we conducted a crowd-sourced annotation study via Amazon Mechanical Turk (AMT) on the top-10 retrievals per query, for $N$ ($N=50$ for UIs and 100 for floorplans) randomly chosen queries outside the training set. 10 turkers were asked to indicate the structural relevance of each of the top-10 results per query, without any specific instructions on what a structural comparison means. A result was considered relevant if at least 6 turkers agreed. For details on the AMT study, please see the supplementary material. 

We observe that LayoutGMN better matches humans' notion of structural similarity. \cite{manandharlearning} performs better than the IoU metric on floorplan data (+3.5\%) on the top-1 retrievals and is comparable to IoU metric on top-5 and top-10 results. On UI layouts, the IoU metric is judged better by turkers than \cite{manandharlearning}. U-Net fails to retrieve structurally similar results as it overfits on the small amount of training data, and relies more on image pixels due to its convolutional structure. LayoutGMN outperforms other methods by at least 1\%  for all $k$, on both datasets. The precision scores on floorplans (bottom-set) are lower than on UI layouts perhaps because they are easier to compare owing to smaller set of semantic elements than UIs and turkers tend to focus more on the size and boundary of the floorplans in additional to the structural arrangements. We believe that when a lot of semantics are present in the layouts and are scattered (as in UIs), the users tend to look at the overall structure instead of trying to match every single element owing to reduced attention-span, which likely explains higher scores for UIs.

\vspace{-10pt}

\paragraph{\textbf{Overlap@k} score.}
%\textbf{\textbf{Overlap@k} score}: 
We propose another measure to quantify the stability of retrieved results: the \emph{Overlap@k} score, or \emph{Ov@k} for short. 
%\agp{
The intuition behind \emph{Ov@k} is to quantify the consistency of retrievals for any similarity metric, by checking the number of similarly retrieved results for a query and its top-1 result. The higher this score, the better the retrieval consistency, and thus, higher the retrieval stability.
%}
Specifically, if $Q_{1}$ is a \emph{set} of queries and $Q_{1}^{top1}$ the \emph{set} of top-1 retrieved results for every query in $Q_{1}$, then
%
\begin{equation}
\label{eqn:overlap_formula}
Ov@k(Q_{1},Q_{1}^{top1}) = \frac{1}{k|Q_{1}|} \sum_{\substack{q_{m} \in Q_{1} \\ q_{p}= top1(q_{m})}} \sum_{j=1}^{k} (L_{mj} \land L_{pj}), 
\end{equation}
%
where $L_{ij}$ is the $j^{th}$ ranked result for the query $q_{i}$, and $\land$ is the logical AND. Thus, ($L_{mj}$ $\land$ $L_{pj}$) is 1 if the $j^{th}$ result for query $q_{m}$ $\in$ $Q_{1}$ and query $q_{p}$ = top1($Q_{1}$)$ \in$ $Q_{1}^{top1}$ are the same. 
\emph{Ov@k} measures the ability of the layout similarity metric to replicate the distance field implied by a query by its top-ranked retrieved result. 
%In other words, retrieval stability can be measured by checking the consistency of retrievals for many (q$_{m}$, q$_{p}$) pairs. 
The score makes sense only when the ranked results returned by a layout similarity tool are deemed reasonable, as assessed by the \emph{P@k} scores. 

\input{Tables/overlap_scores} 

Table \ref{tab:overlap_table} shows the \emph{Ov@k} scores with $k=5,10$ for IoU, GCN-CNN \cite{manandharlearning}, and LayoutGMN on 50 such pairs. On UIs (first three rows), IoU metric has a slightly higher \emph{Ov@5} score (+0.6\%) than LayoutGMN. Also, it shares the largest \emph{P@5} score with LayoutGMN, indicating that IoU metric has slightly better retrieval stability for the top-5 results. However, in the case of \emph{Ov@10}, LayoutGMN has a higher score (+0.4\%) than the IoU metric and also has a higher \emph{P@10} score than the other two methods, indicating that when top-10 retrievals are considered, LayoutGMN has slightly better consistency on the retrievals. 

As for floorplans (last three rows), Table \ref{tab:precision_scores} already shows that LayoutGMN has the best \emph{P@k} scores. This, coupled with a higher \emph{Ov@k} scores, indicate that on floorplans, LayoutGMN has better retrieval stability. In the supplementary material, we show qualitative results on the stability of retrievals for the three methods.

\vspace{-10pt}

\paragraph{Classification accuracy.}
%\textbf{Classification accuracy}: 
We also measure the classification accuracy of test-triplets as a sanity check. However, such a measure alone is not a sufficient one for correctness of a similarity metric employed in information retrieval tasks \cite{manning2008evaluation}. We present it alongside \emph{P@k} and \emph{Ov@k} scores for a broader, informed evaluation, in Table \ref{tab:classification_acc}. 
\input{Tables/classification_acc}
Since user annotations are expensive and time consuming (and hence the motivation to use IoU metric to get weak training labels), we only get user annotations on 452 triplets for both UIs and floorplans, and the last column of Table \ref{tab:classification_acc} reflects the accuracy on such triplets. LayoutGMN outperforms all the baselines by atleast 1.32\%, on triplets obtained using both, IoU metric and user annotations.

\subsection{Fully-connected vs. Adjacency Graphs}
\label{sec:full_vs_adj_graphs}
\begin{figure}[t!]
\centering
\includegraphics[width=\linewidth, height=0.35\linewidth]{Figures/adj_graphs_rets.png}
\vspace{-1.25em}
\caption{Retrieval results for the bottom-left query in Fig \ref{fig:ui_fp_rets}, when adjacency graphs are used. We observe, on most of the queries, that the performance of LayoutGMN improves, but degrades in the case of GCN-CNN \cite{manandharlearning} on floorplan data.}
\label{fig:fc_vs_adj_graphs}
\end{figure}
Following \cite{manandharlearning}, we employed fully connected graphs for our experiments until now and observed that such graphs are a good design for training graph neural networks for learning structural similarity. We also performed experiments using adjacency graphs on GCN-CNN \cite{manandharlearning} and LayoutGMN, and observed that, for floorplans (where the graph node count is small), the quality of retrievals improved in the case of LayoutGMN, but degraded for GCN-CNN. This is mainly because GCN-CNN obtains independent graph embeddings for each input graph and when the graphs are built only on adjacency connections, some amount of global structural prior is lost. On the other hand, GMNs obtain better contextual embeddings by now matching the sparsely connected adjacency graphs, as a result of narrower search space; for a qualitative result using adjacency graphs, see Figure \ref{fig:fc_vs_adj_graphs}. However, for UIs (where the graph node count is large), the elements are scattered all over the layout, and no one heuristic is able to capture adjacency relations perfectly. The quality of retrievals for both the networks degraded when using adjacency graphs on UIs. More results can be found in the supplementary material. %\matt{not sure what the takeaway in this paragraph is; what are we trying to learn?}

\subsection{Ablation Studies on Structural Representation}
\label{sec:ablation_studies}

To evaluate how the node and edge features in our layout representation contribute to
network performance, we conduct an ablation study by gradually removing these features.
Our design of the initial representation of the layout graphs (Sec \ref{sec:layout_graph_extraction}) are well studied in prior works on layout generation \cite{gadi2020read, li2019grains}, visual reasoning, and relationship detection tasks \cite{guo2019aligning, yao2018exploring, manandharlearning}. As such, we focus on analyzing LayoutGMN's behavior when strong structural priors viz., the edges, box positions, and element semantics, are ablated. %\matt{we should give some more motivation why this is a good ablation. normally, ablation would remove features we proposed, but this description seems to be closer to robustness to noise.}

\vspace{-10pt}

\paragraph{Graph edges.}
%\textbf{Graph edges:}
%\rz{
Removing graph edges results in loss of structural information, with only the attention-weighted node update (Eq.~\ref{eqn:node_update}) taking place. When the number of graph nodes is small, e.g., for floorplans, edge removal does not lead to random retrievals, but the retrieved results are poorer compared to when edges are present; see Table \ref{tab:ablation_quant}.%}
%Naturally, the structure encoding is lost in both, the query and the database sample, leading to random retrievals; see first row of Figure \ref{fig:ablation}.

\vspace{-10pt}

\paragraph{Effect of box positions.}
%
%\textbf{Effect of box positions:}
The nodes of the layout graphs encode both the absolute box positions and the element semantics. When the position encoding information is withdrawn, arguably, the most important cue is lost. The resulting retrievals from such a poorly trained model, as seen in the second row of Table \ref{tab:ablation_quant}, are noisy as semantics alone do not provide enough structural priors.

\vspace{-10pt}

\paragraph{Effect of node semantics.}
%
%\textbf{Effect of node semantics:}
Next, when the box positions are preserved but the element semantics are not encoded, we observe that the network slowly begins to understand element comparison guided by the position info, but falls short of understanding the overall structure information, see Table \ref{tab:ablation_quant}.
%
LayoutGMN takes into account all the above information returning structurally sound results (Table \ref{tab:precision_scores}), even relative to the IoU metric. %Qualitative results are provided in the supplementary material.% (last row in Figure \ref{fig:ablation}).

\input{Tables/ablation_quant}

\subsection{Attention-based Layout Label Transfer}
\label{sec:application}

We present {\em layout label transfer\/}, via attention-based structural element matching, as a natural application of LayoutGMN. Given a source layout image $I_{1}$ with known labels, the goal is to transfer the labels to a target layout $I_{2}$. A straight-forward approach to establishing element correspondence is via maximum area/pixel-overlap matching for every element in $I_{2}$ with respect to all the elements in $I_{1}$. However, this scheme is highly sensitive to element positions within the two layouts. Moreover, raster-alignment (via translations) of layouts is non-trivial to formulate when the two layout images have different boundaries and structures. LayoutGMN, on the other hand, is robust to such boundary variations, and can be directly used to obtain element-level correspondences using the built-in attention mechanism that provides an attention score for every element-level match. Specifically, we use a \emph{pretrained} LayoutGMN which is fed with two layout graphs, where the semantic encoding of all nodes is set to a vector of ones. 

As shown in Figure \ref{fig:label_transfer}, the \emph{pretrained} LayoutGMN is able to find the correct labels despite masking the semantic information at the input. Note that when semantic information is masked at the input, such a transfer can not be applied to any two layouts. It is limited by a weak/floating alignment of $I_{1}$ and $I_{2}$, as seen in Figure \ref{fig:label_transfer}.  

\begin{figure}[!t]
\centering
\includegraphics[width=0.95\linewidth, height=0.25\linewidth]{Figures/label_transfer.png}
\vspace{-0.5em}
\caption{Element-level label transfer results from a source image $I_{1}$ to a target image $I_{2}$, using a \emph{pretrained} LayoutGMN vs.~maximum pixel-overlap matching. LayoutGMN predicts correct labels via attention-based element matching.} %Note that in this experiment, the semantics were masked on the input graphs, as well as layout images.}
\label{fig:label_transfer}
\vspace{-0.5em}
\end{figure}



%\begin{figure*}[]
%\centering
%\includegraphics[width=\linewidth, height=0.4\linewidth]{Figures/progressive_ret.pdf}
%\label{fig:progressive_ret}
%\vspace{-0.5em}
%\caption{Retrieval stability when a Floorplan query has been progressively modified (clock-wise from top-left)}
%\end{figure*}

\iffalse
% comment
Figure \ref{fig:ablation} shows qualitative results on top-5 retrieved results for a given query when these structural priors in the training graphs are gradually removed.

\begin{figure}[!t]
\centering
\includegraphics[width=\linewidth, height=0.6\linewidth]{Figures/ablation_studies.pdf}
\vspace{-0.5em}
\caption{Top-5 retrieved results for a given query when structural priors (edges, box positions, and element semantics) are gradually removed from the input graphs.}
\label{fig:ablation}
\end{figure}
% finish commenting
\fi


==> LayoutGMN-CVPR'21/6-conclusions.tex <==
\section{Conclusion, limitation, and future work}
\label{sec:conclusions}

%With the advent of large-scale layout datasets, analysing and organizing layout data becomes crucial, where the first step is to develop an effective means to compare layouts. 
We present the first deep neural network to offer both metric learning of structural layout similarity and structural matching between layout elements. Extensive experiments demonstrate that our metric best matches human judgement of structural similarity for both floorplans and UI designs, compared to all well-known baselines.

The main limitation of our current learning framework is the requirement for strong supervision, which justifies, in part, the use of the less-than-ideal IoU metric for network training. An interesting future direction is to combine few-shot or active learning with our GMN-based triplet network, e.g., by finding ways to obtain small sets of training triplets that are both informative and diverse~\cite{kumari2020}.
Another limitation of our current network is that it does not learn {\em hierarchical\/} graph representations or structural matching, which would have been desirable when handling large graphs.
%
%In addition, the graph embedding space learned by LayoutGMN may be worth a closer examination to assess its potential for generative modeling. %Finally, we would like to explore applying our learning framework to other, more complex graph structured data.

==> LayoutGMN-CVPR'21/Tables/ablation_quant.tex <==
%\begin{figure*}[h]
\begin{table}[!t]
\centering
\begin{tabular}{|c|c|c|c|c|c|}
\hline
\multirow{2}{*}{Structure encoding with} & \multicolumn{3}{c|}{Precision@k (\%)}\\
%\cline{2-7}
 & k=1 ($\uparrow$) & k=5 ($\uparrow$)& k=10 ($\uparrow$)\\
\hline
No edges &30 &16.39 &11.3\\
\hline
No box positions &15 & 7.2&5.4\\
\hline
No node semantics &24 & 11.2&8.4\\
\hline
\end{tabular}
\vspace{-0.5 em}
\caption{Precision@K scores for ablation studies on structural encoding of floorplan graphs. The setup for crowd-sourced relevance judgements via AMT is the same as in Table \ref{tab:precision_scores}, on the same set of 100 randomly chosen queries.}
\label{tab:ablation_quant}
\vspace{-15pt}
\end{table}
%\vspace{-2 em}
%\end{figure*}


==> LayoutGMN-CVPR'21/Tables/classification_acc.tex <==
%\begin{figure*}[h]
\begin{table}[!t]
\centering
\begin{tabular}{|c|c|c|c|c|c|}
\hline
\multirow{2}{*}{Method} & \multicolumn{2}{c|}{Test Accuracy on Triplets}\\
%\cline{2-7}
 & IoU-based ($\uparrow$) & User-based ($\uparrow$)\\
\hline
Graph Kernel \cite{fisher2011characterizing} & 90.09 & 90.73\\
\hline
U-Net \_Triplet \cite{ronneberger2015u} &96.67 &93.38 \\
\hline
GCN-CNN\_Triplet \cite{manandharlearning} &  96.45& 94.48 \\
\hline
LayoutGMN & \textbf{98.96}& \textbf{95.80}\\
\hline\hline
Graph Kernel \cite{fisher2011characterizing} & 92.07 & 95.60\\
\hline
%U-Net \cite{ronneberger2015u} & - & - & & &\\
%\hline
U-Net \_Triplet \cite{ronneberger2015u} & 93.01& 91.00\\
\hline
%GCN-CNN \cite{manandharlearning} & - & - & & &\\
%\hline
GCN-CNN\_Triplet \cite{manandharlearning} &  92.50& 91.8\\
\hline
LayoutGMN & \textbf{97.54}& \textbf{97.60}\\
%\hline
%IoU & 100 & 98.20 \\
%\hline\hline
%GCN-CNN\_Triplet \cite{manandharlearning} &  & \\
%\hline
%LayoutGMN & \textbf{}& \textbf{}\\
\hline
\end{tabular}
\vspace{-0.2 em}
\caption{Classification accuracy on test triplets obtained using IoU metric (IoU-based) and annotated by users (User-based). The first set of comparisons is for UI layouts, followed by floorplans.}
\label{tab:classification_acc}
\end{table}
%\end{figure*}


==> LayoutGMN-CVPR'21/Tables/overlap_scores.tex <==
\begin{table}[!t]
\centering
\begin{tabular}{|c|c|c|c|c|c|}
\hline
\multirow{2}{*}{Method} & \multicolumn{2}{c|}{Overlap@k (\%)}\\
%\cline{2-7}
 & k=5 ($\uparrow$) & k=10 ($\uparrow$)\\
\hline
IoU Metric & \textbf{50.6} &49.4\\
\hline
GCN-CNN\_Triplet \cite{manandharlearning} &46.8 &45.6\\
\hline
LayoutGMN & 49.8 &\textbf{49.8}\\
\hline\hline
IoU Metric & 30.42&30.8\\
\hline
GCN-CNN\_Triplet \cite{manandharlearning} & 43.2 &46.8\\
\hline
LayoutGMN & \textbf{47.6} &\textbf{50.8}\\
\hline
\end{tabular}
\vspace{0.5 em}
\caption{Overlap scores for checking the consistency of retrievals for a query and its top-1 retrieved result, over 50 such pairs. The first set of three rows are for UI layouts, followed by floorplans.}
\label{tab:overlap_table}
\end{table}

==> LayoutGMN-CVPR'21/Tables/precision_scores_table.tex <==
%\begin{figure*}[h]
\begin{table}[!t]
\centering
\begin{tabular}{|c|c|c|c|c|c|}
\hline
\multirow{2}{*}{Method} & \multicolumn{3}{c|}{Precision@k (\%)}\\
%\cline{2-7}
 & k=1 ($\uparrow$) & k=5 ($\uparrow$)& k=10 ($\uparrow$)\\
\hline
Graph Kernel \cite{fisher2011characterizing} &33.33 &15.83 &11.46\\
\hline
U-Net \_Triplet \cite{ronneberger2015u} &27.08 & 10.83&7.92\\
\hline
IoU Metric &43.75 & \textbf{22.92}&14.38\\
\hline
GCN-CNN\_Triplet \cite{manandharlearning} & 39.6&17.1 &13.33\\
\hline
LayoutGMN & \textbf{47.91}& \textbf{22.92} &\textbf{15.83}\\
\hline\hline
Graph Kernel \cite{fisher2011characterizing} &27.27&15.15 &12.42\\
\hline
U-Net \_Triplet \cite{ronneberger2015u} &28.28 &18.18 &15.05\\
\hline
IoU Metric &33.84 & 24.04&17.48\\
\hline
GCN-CNN\_Triplet \cite{manandharlearning} &37.37 & 22.02&17.02\\
\hline
LayoutGMN & \textbf{38.38}& \textbf{25.35} &\textbf{21.21}\\
\hline\hline
\end{tabular}
\vspace{-0.25 em}
\caption{Precision scores for the top-k retrieved results obtained using different methods, on a set of randomly chosen UI and floorplan queries. The first set of five comparisons is for UI layouts, followed by floorplans.}
\label{tab:precision_scores}
\end{table}
%\end{figure*}

